ARFT: A Synchronized Multimodal RF-Acoustic Dataset for Positioning in Distributed Environments

This paper documents the acoustic-radio fusion in Techtile (ARFT) dataset, a synchronized measurement campaign for distributed wireless sensing and positioning in the Techtile testbed. Ultrasonic and radio frequency (RF) signals are simultaneously transmitted and captured at multiple positions in a 2D spatial grid inside the Techtile testbed. Each acquisition cycle corresponds to one rover stop, one position sample, one acoustic recording and one RF snapshot. The RF modality is recorded as per-host pilot measurements and released as channel state information (CSI) tensors for 42 antennas mounted at the ceiling of the room. The acoustic chirp is recorded with 91 synchronized microphones and transmitted by a synchronized quasi omni-directional speaker. The campaign spans 5011 spatial position samples spanning a 5.57 m by 2.89 m area with complete RF and acoustic data. We detail how the measurements are recorded, quantify per-experiment coverage, describe the RF and acoustic data contents, and explain how the aligned modalities support RF-only, acoustic-only, and joint positioning workflows. Furthermore, a static acoustic positioning pipeline that performs anchor selection, pulse-compression ranging, and least squares (LS) localization is elaborated.

==> definitions/def-colors.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%% COLORS FOR TIKZ %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\definecolor{color1}{HTML}{1b9e77}
\definecolor{color2}{HTML}{d95f02}
\definecolor{color3}{HTML}{7570b3}
\definecolor{color4}{HTML}{e7298a}
\definecolor{color5}{HTML}{66a61e}
\definecolor{color6}{HTML}{e6ab02}
\definecolor{color7}{HTML}{a6761d}
\definecolor{color8}{HTML}{666666}
%%%%%%%%%%%%%%%%%%%%%%%%%%%% COLORS FOR TIKZ %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%% DEFINE YOUR OWN COLORS HERE %%%%%%%%%%%%%%%%%%%
% you can use \colorlet to make synonyms, so you can use your own naming conventions
\colorlet{AMBgreen}{color1}
\colorlet{AMBdarkgreen}{color1}
\colorlet{AMBlightgreen}{color1}
\definecolor{darkgray176}{RGB}{176,176,176}

==> definitions/def-tikz.tex <==
\usepackage{tikz}
\usepackage{pgfplots}   % needed regardless of exteralization
\pgfplotsset{compat=newest}
%% the following commands are needed for some matlab2tikz features
\usetikzlibrary{plotmarks}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{arrows}
\usetikzlibrary{calc,fadings,decorations.pathreplacing}
\usetikzlibrary{fit,backgrounds}  % for the fit of boxes


\newcommand{\tikzxmark}{%
\tikz[scale=0.23] {
    \draw[line width=0.7,line cap=round] (0,0) to [bend left=6] (1,1);
    \draw[line width=0.7,line cap=round] (0.2,0.95) to [bend right=3] (0.8,0.05);
}}
\newcommand{\tikzcmark}{%
\tikz[scale=0.23] {
    \draw[line width=0.7,line cap=round] (0.25,0) to [bend left=10] (1,1);
    \draw[line width=0.8,line cap=round] (0,0.35) to [bend right=1] (0.23,0);
}}
\newcommand{\yes}{\protect\tikzcmark}
\newcommand{\no}{} %\protect\tikzxmark

						% Tikz
\usetikzlibrary{shapes,arrows,fit,positioning}
\usetikzlibrary{shapes}
\usetikzlibrary{spy}
\usetikzlibrary{circuits}
\usetikzlibrary{arrows}

%%%%%%%%%%%% MAKE FIGURES MORE UNIFORM %%%%%%%%%%%%
\pgfplotsset{
    every axis/.append style={
        title style={draw=none},
        label style={font=\small},
        legend style={
            fill opacity=0.8,
            nodes={scale=0.8, transform shape}, {draw=none}
        },
        tick align=outside,
        tick pos=left,
        x grid style={darkgray176},
        xtick style={color=black},
        y grid style={darkgray176},
        ytick style={color=black},
        grid=both,
    },
    every axis plot/.append style={
        line width=2.0pt,
    },
}


\newlength{\plotWidth}		% a parameter for scaling the TikZ plots
\tikzset{%
  >=latex,
  inner sep=0pt,%
  outer sep=2pt,%
  mark coordinate/.style={inner sep=0pt,outer sep=0pt,minimum size=3pt,
  fill=black,circle}%
}

==> sections/how-to-use.tex <==
\section{How To Use this template and best practices}

\begin{itemize}
    \item Make use of the \textbf{glossaries} package to conveniently expand abbreviations in the correct manner. The abbreviations are located in \texttt{abbr.tex}.
    \item Use \textbf{booktabs} 
    \item Use distinct and descriptive labels to reference figures/tables/...
    \item Use \texttt{cref} opposed to just \texttt{ref}.
    \item Use plain old CSV to transform eps/png/pdf figures to \textbf{tikz} figures which gives us more control over the aesthetics of the figures (coherent coloring scheme, font size, font family, size,...)
    \item Make use of the \texttt{defineauthors} command (see \texttt{main.tex}) to use inline comments. Example: \gilles{example comment}.
\end{itemize}
